Extracting Protocol Format as State Machine via Controlled Static Loop Analysis

Reverse engineering of protocol message formats is critical for many security applications. Mainstream techniques use dynamic analysis and inherit its low-coverage problem -- the inferred message formats only reflect the features of their inputs. To achieve high coverage, we choose to use static analysis to infer message formats from the implementation of protocol parsers. In this work, we focus on a class of extremely challenging protocols whose formats are described via constraint-enhanced regular expressions and parsed using finite-state machines. Such state machines are often implemented as complicated parsing loops, which are inherently difficult to analyze via conventional static analysis. Our new technique extracts a state machine by regarding each loop iteration as a state and the dependency between loop iterations as state transitions. To achieve high, i.e., path-sensitive, precision but avoid path explosion, the analysis is controlled to merge as many paths as possible based on carefully-designed rules. The evaluation results show that we can infer a state machine and, thus, the message formats, in five minutes with over 90% precision and recall, far better than state of the art. We also applied the state machines to enhance protocol fuzzers, which are improved by 20% to 230% in terms of coverage and detect ten more zero-days compared to baselines.

==> autopilot.tex <==

\section{Application to Autopilot Systems}\label{app:ardupilot}



\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figs/pgfuzz}
    \caption{(a) The code that implements the FSM to control a copter to flip. The red underlined variables are inputs from sensors. (b) The FSM we infer from the code.}
    \label{fig:pgfuzz}
\end{figure}

Autopilot systems, such as ArduPilot~\cite{ardupilot},
enables the creation and control of robotic vehicle systems such as copters and planes.
They often use state machines to let a robotic vehicle automatically complete a movement or mission,
such as flip, rotation, and takeoff, to name just a few.
Table~\ref{tab:ardupilot} shows ten FSMs we inferred from the ArduPilot systems, 
including the time cost of FSM inference and the sizes of each inferred FSM.
Figure~\ref{fig:pgfuzz}(a)
shows the code from ArduPilot that automatically controls a copter to flip via an FSM.
The function loop() first checks the initial constraints. If the constraints are satisfied, it enters a loop to run the FSM.
For instance,
Line 14 performs the state transition from the state Roll to the state Recover
when the flip angle, an input to the system, satisfies the constraint
$-9000<\textit{flip\_angle} < 4500$. Otherwise, it stays in the state Roll. 

The code is similar to a parsing loop in protocol parsers except that the inputs are no longer \mreplace{a network message}{from the network} but from different sensors, such as the gyroscope.
Figure~\ref{fig:pgfuzz}(b) shows the FSM we infer from the code. Each state transition is labeled by a constraint.
For instance,
from the FSM, we can conclude that the initial constraint for flipping is 
$\phi_\textup{init}\equiv\phi_0\lor\phi_1\lor\phi_2\lor\phi_3\equiv -4000 < \textit{roll} < 4000 \land \cdots$,
which is inferred from the if-statement at Line 2 of the code snippet.
Also, the constraint for staying in the state Roll is $\phi_\textup{17}\equiv \textit{flip\_angle}\ge 4500 \lor \textit{flip\_angle}  \le -9000$, which is inferred from the if-statement at Line 13.
In terms of security analysis, such FSMs can enhance stateful fuzzing by
finding bugs not only in autopilot systems but also in the fuzzers~\cite{hehe}.


\begin{table}[h]
    \centering
    \footnotesize
    \caption{State machines in ArduPilot.}~\\
    \label{tab:ardupilot}
    \begin{tabular}{r|ccc}
        \toprule
        \textbf{Modes} & \textbf{Time (Seconds)} & \textbf{\# State} & \textbf{\# Transitions} \\
        \midrule
        Copter\_AutoRotate & 10 &7&21\\
        Copter\_Flip             & 15&10&28\\
        Copter\_RTL            &9&14&45\\
        Copter\_SmartRTL   &21&14&76\\
        Copter\_Throw       &12&9&26\\
        Copter\_ZigZag      &19&9&39\\
        Plane\_RTL             &7&4&9\\
        Plane\_TakeOff        &22&7&23\\
        Sub\_MotorDetect  &8&6&19\\
        Rover\_SmartRTL    &8&12&44\\
        \bottomrule
    \end{tabular}
\end{table}


%We leverage the inferred FSM to fuzz ArduPilot via PGFuzz~\cite{kim2021pgfuzz}, which is a recent fuzzer specially designed for autopilot systems.
%As shown in Figure~\ref{fig:pgfuzz}(c),
%PGFuzz provides a set of \mrevise{pre-defined} policies,
%which are mandatory constraints \mdelete{and serve as the ground truth}that ArduPilot cannot violate at runtime.
%These policies are manually created by the developers of PGFuzz based on their understanding of the systems' documents.
%During the fuzzing procedure, PGFuzz randomly changes the inputs to see if any policies \mreplace{could be}{are} violated or if the system could crash.
%Two of the policies are shown in Figure~\ref{fig:pgfuzz}(d), 
%where $\phi_\textup{init}$ stands for the initial constraints of flipping and $\phi_\textup{17}$ is the constraint for staying in the state Roll.
%
%The corresponding constraints inferred by our approach from the code are also shown in Figure~\ref{fig:pgfuzz}(d).
%They are different from the policies in PGFuzz.
%These differences lead to three interesting findings when we fuzz the flipping movement of a copter.
%First,
%when the fuzzer sets \mreplace{$\textit{Roll} = 4300$}{the input $\textit{roll} = 4300$},
%we expect PGFuzz to crash the system as the value does not satisfy the constraint $\phi_\textup{init}$ in \mreplace{the}{our inferred} FSM.
%However, PGFuzz works normally as the value of \textit{Roll} still satisfies PGFuzz's policy.
%After investigation, we confirm that this inconsistency is caused by the incorrect policy $\phi_\textup{init}$ in PGFuzz.





%Second,
%when the fuzzer sets \mreplace{$\textit{Throttle} = 1000$}{the input $\textit{throttle} = 1000$},
%we expect \mreplace{it}{the autopilot system} to work normally 
%as the initial constraints \mrevise{$\phi_\textup{init}$ inferred by us} do not constrain this input.
%However, PGFuzz reports a policy violation as it requires $\textit{throttle} > 1500$.
%We then investigate why we do not obtain the constraint \mrevise{$\textit{throttle} > 1500$} when inferring the FSM.
%The conclusion is that the function init() in the source code misses this constraint. Hence, this is a vulnerability in Ardupilot.
%
%Third,
%when ArduPilot controls a vehicle to flip, reaches the state Roll,
%and the fuzzer sets \mrevise{the input} $\textit{flip\_angle} = 4800$,
%we expect the vehicle to stay in the state Roll
%but ArduPilot reports a policy violation as \mreplace{it}{its policy $\phi_{17}$} requires the value of \textit{flip\_angle} to be in a different range.
%After comparing  PGFuzz's policy and the constraint $\phi_{17}$ produced by ourselves,
%we confirm that the policy in PGFuzz is not correct.

%To sum up, with an inferred FSM,
%we not only find vulnerabilities in autopilot systems but also provide a way to enhance security-support tools like PGFuzz.
%While finding vulnerabilities in autopilot systems directly help them ensure security,
%from the other perspective,
%enhancing security-support tools such as PGFuzz is also important for security analysis.
